Regularized Fingerprinting in Detection and Attribution of Climate Change with Weight Matrix Optimizing the Efficiency in Scaling Factor Estimation

The optimal fingerprinting method for detection and attribution of climate change is based on a multiple regression where each covariate has measurement error whose covariance matrix is the same as that of the regression error up to a known scale. Inferences about the regression coefficients are critical not only for making statements about detection and attribution but also for quantifying the uncertainty in important outcomes derived from detection and attribution analyses. When there is no errors-in-variables (EIV), the optimal weight matrix in estimating the regression coefficients is the precision matrix of the regression error which, in practice, is never known and has to be estimated from climate model simulations. We construct a weight matrix by inverting a nonlinear shrinkage estimate of the error covariance matrix that minimizes loss functions directly targeting the uncertainty of the resulting regression coefficient estimator. The resulting estimator of the regression coefficients is asymptotically optimal as the sample size of the climate model simulations and the matrix dimension go to infinity together with a limiting ratio. When EIVs are present, the estimator of the regression coefficients based on the proposed weight matrix is asymptotically more efficient than that based on the inverse of the existing linear shrinkage estimator of the error covariance matrix. The performance of the method is confirmed in finite sample simulation studies mimicking realistic situations in terms of the length of the confidence intervals and empirical coverage rates for the regression coefficients. An application to detection and attribution analyses of the mean temperature at different spatial scales illustrates the utility of the method.

==> Makefile <==
source := $(wildcard fpweight.tex)
out := $(patsubst %.tex,%.pdf,$(source))
rev := 56a50ce
latest := $(shell git log --format="%h" | head -n 1)
bib := $(wildcard *.bib)

.PHONY: all
all: $(out)

%.pdf: %.tex $(bib)
	@latexmk -pdf $<
#	@latexmk -c

## compare modification with the latest version checked into git
## for comparison of specific commits:
##	latexdiff-vc --git -r old_githash -r new_githash --pdf source.tex
diff:
	latexdiff-vc --git --pdf --force $(source) -r $(rev)

log:
	@git log --pretty=format:"%h by %an at %ar: %s" $(source) | head -n 15

.PNONY: clean
clean:
	rm -rf $(out)\
	  *~ .*~ .\#* .Rhistory *.aux *.bbl *.blg *.out *.log *.toc\
	  *.fff *.fdb_latexmk *.fls *.ttt *diff* *oldtmp*


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
